Specializing Scope Graph Resolution Queries: Extended Edition

To warrant programmer productivity, type checker results should be correct and available quickly. Correctness can be provided when a type checker implementation corresponds to a declarative type system specification. Statix is a type system specification language which achieves this by automatically deriving type checker implementations from declarative typing rules. A key feature of Statix is that it uses scope graphs for declarative specification of name resolution. However, compared to hand-written type checkers, type checkers derived from Statix specifications have sub-optimal run time performance. In this paper, we identify and resolve a performance bottleneck in the Statix solver, namely part of the name resolution algorithm, using partial evaluation. To this end, we introduce a tailored procedural intermediate query resolution language, and provide a specializer that translates declarative queries to this language. Evaluating this specializer by comparing type checking run time performance on three benchmarks (Apache Commons CSV, IO, and Lang3), shows that our specializer improves query resolution time up to 7.7x, which reduces the total type checking run time by 38 - 48%.

==> figures/scope-graphs/definitions.tex <==
\begin{figure}
\begin{adjustbox}{minipage={\linewidth}, padding=1ex, frame, max width = \linewidth}
  \figuresection{Scope Graphs}
  \vspace{-0.5em}
  \begin{align*}
    \renewcommand\arraystretch{1.0}
    \begin{array}{r O l T}
      \hspace{1.3em} \scope & \in & \Scopes  & \hspace{0.1em} scopes \\
                     \datum & \in & \Data    & data \\
    \end{array}
    \hspace{2.9em}
    \begin{array}{r O l T}
      \edgelbl & \in & \Labels  & labels \\
      \edge{\scope}{\edgelbl}{\scope} & \in & \Edges & \hspace{1.2em} edges  \\
    \end{array}
    \\
    \begin{array}{r O l c}
      \SG & := & \SGrep{\scopes \subset \Scopes}{\edges \subset \Edges}{\dataassoc \subset \Scopes \rightharpoonup \Data} & \hspace{-0.5em}
    \end{array}
  \end{align*}
  \vspace{-1em}
  \figuresection{Query Resolution Parameters}
  \vspace{-0.5em}
  \begin{align*}
    \renewcommand\arraystretch{1.0}
    \begin{array}{r O l O l T}
      \pathlbl    & \in     & \PathLabels & \hspace{0.2em} := & \edgelbl \alt \EOP        & extended labels \\
      \re         & \in     & \RE         & \subset & \Labels^\ast                        & label well-formedness regex \\
      \wfd(\cdot) & \subset & \multicolumn{3}{l}{\Data}                                   & data well-formedness predicate \\
      \lblOrd     & \subset & \multicolumn{3}{l}{\PathLabels \times \PathLabels}          & strict partial order on labels \\
      \equivd     & \subset & \multicolumn{3}{l}{\Data \times \Data}                      & data equivalence relation
    \end{array}
  \end{align*}
  \vspace{-0.5em}
  \figuresection{Query Answers}
  \vspace{-0.5em}
  \begin{align*}
    \renewcommand\arraystretch{1.0}
    \begin{array}{r O l O l T}
      \hspace{1.2em} \sgpath & \in & \Paths      & := & \scope \alt \pathseg{\scope}{\edgelbl}{\sgpath}  & \hfill paths \\
                     \Answer & \in & \AnswerSets & =  & \powerset{\Paths}                                & \hspace{5em} environments \\
    \end{array}
  \end{align*}
  \vspace{-1em}
\end{adjustbox}

\caption{Scope Graph Definitions}
\label{fig:scope-graph-definitions}

\end{figure}


==> figures/scope-graphs/path-order.tex <==
\begin{figure}
  \begin{adjustbox}{minipage={\linewidth}, padding=1ex, frame, max width = \linewidth}
	  \setpremisesend{.5ex}
    \figuresection[\fbox{${\lblOrd} \vdash \sgpath \pathOrd \sgpath$}]{Prefix Order on Paths}
    \begin{gather*}
      \inference{
        {\lblOrd} \vdash \sgpath_1 \pathOrd \sgpath_2
      }{
        {\lblOrd} \vdash \pathseg{\scope}{\edgelbl}{\sgpath_1} \pathOrd \pathseg{\scope}{\edgelbl}{\sgpath_2}
      }
      \qquad
      \inference{
        \EOP \lblOrd \edgelbl
      }{
        {\lblOrd} \vdash \scope \pathOrd \pathseg{\scope}{\edgelbl}{\sgpath}
      }
      \\
      \inference{
        \edgelbl \lblOrd \EOP
      }{
        {\lblOrd} \vdash \pathseg{\scope}{\edgelbl}{\sgpath} \pathOrd \scope
      }
      \qquad
      \inference{
        \edgelbl_1 \lblOrd \edgelbl_2
      }{
        {\lblOrd} \vdash \pathseg{\scope}{\edgelbl_1}{\sgpath_1} \pathOrd \pathseg{\scope}{\edgelbl_2}{\sgpath_2}
      }
    \end{gather*}
  \end{adjustbox}

  \caption{Prefix Order on Paths}
  \label{fig:path-prefix-order}
\end{figure}


==> figures/scope-graphs/resolution-algorithm-new.tex <==
\begin{figure*}
  \begin{boxedalgorithm}
    \Input{\hspace{0.3em}$\SG, \scope, \re, \wfd, \lblOrd$}
    \Output{\hspace{0.3em}\ResolveAll{$\scope, \re$}}
    %\Fn{\Resolve{$\SG, \scope, \re, \wfd, \lblOrd, \equivd$} \withRT\AnswerSets}{
      \vspace{\localfundefskip}
      \LocalFn{\ResolveAll{$\sgpath,\re'$} \withRTNR\AnswerSets}{%
        \ResolveL{$\sgpath, \rehead{\re'} \cup \setOf{ \EOP \alt \reeps \in \langOf{\re'}}, \re'$}
      }%
      \EndLocalFnDef
      \LocalFn{\ResolveL{$\sgpath, \pathlbls, \re'$} \withRTNR\AnswerSets}{%
        $\mathrel{\bigcup}_{\pathlbl \in \maxOf{\pathlbls}}$ \ResolveLl{$p, \smallerOf{\pathlbls}{\pathlbl}, \pathlbl, \re'$}
      }
      \vspace{-0.5em}
      \EndLocalFnDef
      \Fn{\ResolveLl{$\sgpath, \pathlbls, \pathlbl, \re'$} \withRTNR\AnswerSets}{%
        $E_{\pathlbls}$ := \ResolveL{$\sgpath, \pathlbls, \re'$}\;
        \Ternary{$E_{\pathlbls} \neq \emptyset$}{\Return $E_{\pathlbls}$}{\Return \Resolvell{$p, \pathlbl, \re'$}}
      }
      %\EndLocalFnDef
      \LocalFn{\Resolvell{$\sgpath, \pathlbl, \re'$} \withRTNR\AnswerSets}{%
        \Ternary{$\pathlbl = \EOP$}{\ResolveEOP{$\sgpath$}}{\Resolvel{$\sgpath, \pathlbl, \re'$}}%
      }
      \LocalFn{\ResolveEOP{$\sgpath$} \withRTNR\AnswerSets}{%
        $\setOf{ \sgpath \alt \wfd(\assocOf{\target{\sgpath}}) }$
      }%
      \EndLocalFnDef
      \LocalFn{\Resolvel{$\sgpath, \edgelbl, \re'$} \withRTNR\AnswerSets}{%
        $\mathrel{\bigcup} \setOf{ \ResolveAll{$\pathseg{\sgpath}{\edgelbl}{s'}, \derive{l}\re'$} \alt \scope' \in \getEdgesOf{\target{\sgpath}}{\edgelbl}, \scope' \notin \sgpath}$
      }%
      \EndLocalFnDef
      %\Return \ResolveAll{$\scope, \re$}
    %}
  \end{boxedalgorithm}

  \caption{Query Resolution Algorithm}
  \label{fig:query-resolution-algorithm}
\end{figure*}

==> sections/01-partial-evaluation.tex <==
\section{Partial Evaluation for DSL Interpreters}
\label{sec:partial-evaluation}

In this section, we provide a brief introduction to partial evaluation, and explain why we think it is especially beneficial for declarative languages.
Partial evaluation was popularized by \citenamed{Futamura82}.
A program might be seen as a function from inputs to an output $O$.
Some of these inputs may be known statically ($S$), while some of them may vary per invocation ($D$).
Then, the signature of a program looks as follows:
\[
  \mathsf{prog} : S \times D \to O
\]
A \emph{specializer} takes such a program and its static input, and returns a \emph{residual program} $\mathsf{prog}_{S} : D \to O$.
When generating $\mathsf{prog}_{S}$, it performs the part of the computation that does not depend on $D$, making $\mathsf{prog}_{S}$ generally faster than $\mathsf{prog}$.


\subsection{Partial Evaluation for Interpreters}

This pattern can easily be applied to programming languages.
In that case, $\mathsf{prog}$ is an interpreter that evaluates the semantics of a program (its static input $S$) with respect to some arguments $D$.
The residual program is essentially a compiled version of $S$.
This is called the \emph{first Futamura projection}.

Specialization is generally only beneficial when a program is executed multiple times.
However, Futamura argues that specializing an interpreter to a program may already be beneficial when executing the program once, as programs may repeatedly evaluate a particular piece of code.
Specializing repeatedly executed program fragments removes the interpretation overhead, which might outweigh the run time costs of compilation.
This effect becomes stronger when the computational complexity of interpreting particular language constructs is high.
That is, the more overhead an interpreter introduces, the more beneficial specialization will be.

Declarative languages are languages in which a user specifies intent rather than procedure.
The logic to compute a result that corresponds to the intent is then implemented in the back-end (i.e., its interpreter) of the language.
Thus, a declarative language moves part of the complexity of a problem from the program or programmer to its interpreter.

Having a complex back-end means that declarative languages are susceptible to introducing relatively more run time overhead compared to non-declarative languages.
Interpreters of imperative languages might have to execute non-trivial algorithms in order to evaluate a program.
For that reason, partial evaluation might be relatively beneficial for declarative languages.


\subsection{Multi-Stage Partial Evaluation}

However, this may be easier said than done.
As the semantics of a declarative language can be intricate, finding a specializer that compiles the full language can be challenging.
Instead, it might be possible to find a subset of language constructs that are particularly complex to evaluate.
Specializing only those constructs will then still yield significant performance gain, but avoid the complexity of full compilation.

To formalize this, we generalize to \emph{multi-stage} partial evaluation.
For simplicity, we present a two-stage variant, but it can easily be generalized to an arbitrary number of stages.
First, recall the definition of an interpreter:
\[
  \mathsf{interp}: P \times D \to O
\]
where $P$ is the interpreted program with input $D$ and result $O$.
Now, suppose we can divide $P$ into two components:
\[
  P \equiv P_0 \uplus P_1
\]
where $P_0$ is the part of the program to which the interpreter will be specialized at the first stage, and $P_2$ at the second stage.
The $\uplus$ symbol is chosen to indicate that these groups can be (mutually) embedded in an actual AST.
Now, we can define two partial specializers as follows:
\begin{align*}
  \mathsf{spec}_0&: (P_0 \uplus P_1 \times D \to O) \times P_0 \uplus P_1 \to P_I \uplus P_1 \\
  \mathsf{spec}_1&: P_I \uplus P_1 \to (D \to O)
\end{align*}
where $P_I$ is an interpreter, specialized to $P_0$ only.
Thus, $P_I$ complemented with $P_1$ represents a program $D \to O$.
The parts of the interpreter that interprets $P_1$ are still present in $P_I$.
Those are eliminated by $\mathsf{spec}_1$, yielding an executable.

However, it is not necessary to apply the second specializer.
Instead, one could define an interpreter for the partially specialized program as follows:
\[
  \mathsf{interp}_1: P_I \uplus P_1 \times D \to O
\]
Writing such an interpreter might be easier than the corresponding specializer, as operations on $P_1$ and $D$ can be interleaved.
Still, when constructs with complex semantics are included in $P_0$, this approach will give significant speedup.

% When the evaluation of language constructs with high evaluation complexity is specialized away in the first phase (i.e., the part of the program with high evaluation overhead are in $P_0$), we have essentially transformed a high-overhead interpreter ($\mathsf{interp}$) to a low-overhead one ($\mathsf{interp}_1$).


\subsection{Heterogeneous Specialization}

Typically, an interpreter of a (declarative) language is written in a different language.
This raises the question in which language $P_I \uplus P_0$ is represented.
The original language might not always be a good choice when it (being declarative) lacks constructs to express the remaining part of the interpreter.
However, the language of the interpreter might not be a good choice either, as there it still contains a part of the original program $P_1$.
Instead, a third option is to define an intermediate language that is similar to the language of $P$, but allows embedding the partially specialized interpreter.
We call this approach `heterogeneous specialization'.

This approach looks similar to, but is not necessarily equal to, compiling to an intermediate language.
In our view, compiling is merely transforming a program, leaving the overall structure intact.
On the other hand, we regard specialization as (partially) interpreting the subject program.
That is, a specializer should lift an essential part of the complexity of the interpreter to compile time.

% TODO: per feedback Soham, could we provide an example here?


\subsection{Application to Statix}

In the remainder of the paper, we explain how we apply this pattern to Statix.
First, we explain that interpreting a particular language construct (scope graph queries) is computationally complex (that is, $\mathsf{interp}$ has significant overhead).
Therefore, we specialize our `interpreter' (the query resolution algorithm embedded in the Statix solver), to these queries (i.e., the queries are in $P_0$, optimized away by $\mathsf{spec}_0$).
These specialized queries ($P_I$) cannot be represented in either Statix itself or Java (the language in which the solver is written).
Thus, we introduce an intermediate language to express those (i.e., the specialization is heterogeneous).
For this language, we provide an interpreter.
This low-overhead interpreter, integrated in the Statix solver, yields $\mathsf{interp}_1$.


==> sections/02-graph-query-resolution.tex <==
\section{Resolving Queries in Scope Graphs}
\label{sec:query-resolution-in-scope-graphs}

In this section, we explain how scope graphs can be used to model name binding, and how references in scope graphs are resolved.

\subsection{Scope Graphs}
\label{subsec:scope-graphs}

\input{figures/scope-graphs/example}

In this section, we introduce scope graphs using the example in \cref{fig:scope-graph-example}.
This figure shows a program in Language with Modules (LM, introduced by \citenamed{NeronTVW15}).
The scope graph contains nodes, which model scopes and declarations, and labeled directed edges.
The scope $s$ models the global scope, in which top-level declarations are made.
For example, $s_A$ models the declaration of module \texttt{A} in the global scope.
The name of the module \id{A} is associated with $s_A$ as datum.
In addition, to indicate that it represents a module, a \lblMOD label is used on the edge that connects $s_A$ to $s$.
At the same time, $s_A$ models the scope of the body of module \texttt{A} as well.
Thus, as the global scope $s$ is the \emph{lexical parent} of the body of module \texttt{A}, there is a \lblLEX-labeled edge from $s_A$ to $s$.
Moreover, the declaration of module \texttt{B}, which syntactically appears in the body of module \texttt{A}, is done in $s_A$.
Similar to the declaration of module \texttt{A}, $s_B$ has its name \id{B} as datum, is connected to $s_A$ with an \lblMOD-labeled edge and has a parent edge back to $s_A$.
Scope $s_x$ models the declaration of the variable \texttt{x}.
The type of \texttt{x} is indicated by the datum of scope $s_{T(x)}$, which is connected to $s_x$ using a \lblTYPE edge.
For module \texttt{C} and definition \texttt{f}, similar declarations are made.
Because module \texttt{C} imports module \texttt{A}, there is an \lblIMPORT-labeled edge from $s_C$ to $s_A$.
This ensures that declarations in $s_A$ are reachable from $s_C$.
Finally, scope $s_b$ models the body of the function \texttt{f}.
Therefore, it has a \lblLEX edge to $s_C$ (its lexical context) and a declaration for the parameter \texttt{x}.

In the program, there are a number of references, each indicated with a color.
In the scope graph, the resolution paths of their queries are indicated with colored edges.
For example, the reference \coloredref{query-1}{x} resolves to the declaration in the same scope.
This corresponds to the intuition that it is bound by the \texttt{\textbf{fun}} formal argument specifier.
The qualified reference \texttt{\coloredref{query-2}{B}.\coloredref{query-3}{x}} is modeled using two queries.
The first query resolves the qualifier \coloredref{query-2}{B} to $s_B$.
Then, the second part \coloredref{query-3}{x} is resolved relatively to $s_B$, which yields $s_x$.

In the scope graph framework, queries have several parameters that guide their resolution.
We discuss these based on the query for the reference \coloredref{query-2}{B}.
First, there is the \emph{path well-formedness} condition.
This is a regular expression over labels that describes valid paths.
For our example, this would be $\reclos{\lblLEX} \reopt{\lblIMPORT} \lblMOD$.
This encodes that a we are looking for a module declaration (hence the \lblMOD at the end), in a lexical parent of the starting scope, while possible passing through a non-transitive import.
This excludes paths to scopes that are not module declarations, or paths to module declarations that are not in scope.
However, there are paths to $s_A$ and $s_C$ that match this path well-formedness condition as well.
To ensure these paths are not included in the query result, a \emph{data well-formedness} condition is used as the second parameter.
This condition, defined as a unary predicate over datums, is applied to the target scopes of all candidate paths.
For usual reference resolution, this predicate checks whether the datum is equal to the name of the reference.
For example, the query for reference \coloredref{query-2}{B} will only match module declarations with \id{B} as datum, such as $s_B$.
Paths that match both of these conditions are called \emph{reachable}.

When resolving names, it is important to apply shadowing correctly.
For example, assuming the regular expression used to resolve \coloredref{query-1}{x} is $\reclos{\lblLEX} \reopt{\lblIMPORT} \lblVAR$, $s_x$ is a reachable definition as well.
However, $s_{x'}$ is preferred because it `binds closer'.
This is encoded in a third query parameter: the \emph{label order}, which is a partial order on edge labels.
For example, the label order $\lblVAR \lblLE \lblLEX \lblLE \lblIMPORT$ encodes that the query resolution should prefer \lblVAR-labeled edges over edges with a \lblLEX label.
Therefore, the resolution algorithm prefers the path via edge $\pathseg{s_b}{\lblVAR}{s_{x'}}$ over the path via edge $\pathseg{s_b}{\lblLEX}{s_C}$.
Finally, there is a fourth argument: the \emph{data equivalence condition}, expressed as a binary predicate over datums.
This condition acts as a `grouping operator' over reachable paths.
The shadowing based on label orders is only applied within a group.
That is, a path shadows another path only if it is preferred according to the label order \emph{and} the target datums are in the same group.
In typical name resolution queries, the data equivalence condition is simply true (denoted as $\top$) for any pair of data.
However, consider a query that finds all \emph{visible} declarations in $s_b$.
This query would have a data well-formedness predicate that matches all declarations.
However, when paths shadow each other based on labels only, the path to $s_{x'}$ would shadow the path to $s_f$, which is obviously incorrect.
Therefore, such a query would have a data equivalence condition that checks for data (declaration name) equality.
In that case the path to $s_{x'}$ would still shadow the path to $s_x$, but not the path to $s_f$.

\input{figures/scope-graphs/definitions}

We now discuss the formal representation of scope graphs as given in \cref{fig:scope-graph-definitions}.
Scope graphs $\SG$ consist of a collection of scopes, edges and a mapping from scopes to data $\dataassoc$.
The scopes and edges of a scope graph can be retrieved using the $\scopesOf{\SG}$ and $\edgesOf{\SG}$ projections.
In addition, the $\getEdgesOf{\scope}{\edgelbl}$ returns the target scopes of all outgoing edges of $\scope$ with label $\edgelbl$.
Retrieving the datum of a scope is denoted as $\assocEq{\scope}{\datum}$.
The $\re$ query parameter is a regular expression over the alphabet $\Labels$, describing valid paths.
The data well-formedness predicate $\wfd(\cdot)$ identifies matching declarations for a query.
In the text, we usually denote predicates that match a particular name, say $\id{x}$, with $\wfdOf{\id{x}}$.
Regarding shadowing, $\lblOrd$ represent the ordering on labels.
The domain of $\lblOrd$ is enlarged with $\EOP$, which represents the end of a path.
This allows comparing a path with an extension of itself.
For example, with $\EOP \lblLE \lblLEX$, the path $\scope$ is smaller than $\pathseg{\scope}{\lblLEX}{\scope'}$. 
The grouping operator $\equivd$ ensures that shadowing is only applied to equally named declarations.
A query answer $\Answer$ consists of a set of paths $\Paths$, where each path is an alternating sequence of scopes and labels.
Paths are presented in right-recursive style, but we use a left-recursive notation style (i.e., $\pathseg{\sgpath}{\edgelbl}{\scope}$) as well.
We use the $\source{\sgpath} = \scope$ and $\target{\sgpath} = \scope$ projections to retrieve the source and target of a path, respectively.


\subsection{Resolving Queries}
\label{subsec:resolving-queries}

\input{figures/scope-graphs/path-order}

The previous section gave an informal description of query resolution.
A formal resolution calculus is given by \Citenamed[sect. 2]{AntwerpenPRV18}.
In this section, we discuss a subtle but important detail from that resolution calculus, and discuss the resolution algorithm that implements this resolution calculus.

A naive approach to query resolution would be to compute all valid paths, and subsequently do a pairwise comparison between all paths to retain the unshadowed ones.
However, a pairwise comparison of all paths is computationally expensive.
Therefore, the decision was made to define the ordering on paths as a \emph{prefix order}, which means that paths only shadow each other when they have a shared prefix.
For example, given $\lbldef{L_1} \lblLE \lbldef{L_2}$ as label order, $\pathseg{\scope_1}{\lbldef{L_1}}{\scope_1'} \not\pathOrd \pathseg{\scope_2}{\lbldef{L_2}}{\scope_2'}$ when $\scope_1 \neq \scope_2$.
This ordering is made precise in \cref{fig:path-prefix-order}.
In the remainder of this section, we show how this way of ordering can be integrated in the query resolution algorithm, making it more efficient.

\input{figures/scope-graphs/resolution-algorithm}

The resolution algorithm \Resolve of scope graph queries is given in \cref{fig:query-resolution-algorithm}.
It receives a scope graph, an initial scope and the query parameters discussed earlier as arguments, and returns a query answer.
The actual algorithm consists of a few steps, which are each encoded in an inner local function.
The algorithm searches valid paths in one direction, starting at $\scope$.
Therefore, the inner functions have a \emph{path prefix} $\sgpath$ as first argument.

We now discuss these steps one by one.
The \ResolveEOP function checks whether the current path prefix is a valid path for the query.
It does so by checking if the datum associated with the target scope is valid with respect to $\wfd$.
When it is valid, the function will return a singleton set containing $\sgpath$.
Otherwise, it returns an empty set.
The \Resolvel~function has two additional arguments: a label $\edgelbl$ to traverse, and a path well-formedness condition $\re'$.
This condition has the invariant that for any path $\sgpath'$ that starts in $\target{\sgpath}$ and satisfies $\re'$, $\sgpath$ concatenated with $\sgpath'$ satisfies the initial path wellformedness condition $\re$.
The body of this function retrieves all outgoing edges from $\target{\sgpath}$ with label $\edgelbl$.
Then, for each new target scope a \emph{residual query} is executed.
Cyclical path are excluded using the $\scope' \notin \sgpath$ side condition.
This residual query has $\sgpath$ extended with the new edge as prefix.
Its path well-formedness is $\derive{\edgelbl}\re$, which is the \emph{Brzozowski derivative} of $\re$ with respect to $\edgelbl$~\cite{Brzozowski64}.
This retains the invariant discussed above, ensuring query results are well-formed with respect to $\re$.
\Resolvell~receives a path label $\pathlbl$, and based on its value decides the correct function to resolve it with.
Its return value is called a \emph{single-label environment} or \lenv.

To compute a full query answer, the various \lenv's that together form the result should be combined appropriately.
This is implemented by the \ResolveLl~and \ResolveL~functions.
\ResolveLl~receives a path label $\pathlbl$ and a set of other labels $\pathlbls$.
These arguments have the invariant that all labels $\pathlbl'$ in $\pathlbls$ are smaller than $\pathlbl$ with respect to $\lblOrd$.
The function computes the combined environment of all labels in $\pathlbls$ (called an \Lenv) and the \lenv of $\pathlbl$.
Then it applies shadowing by filtering out all paths in \lenv that have a datum equivalent to a datum in \Lenv under $\equivd$ (implemented in \Shadow).
This captures the notion that paths over smaller labels take precedence over paths with a higher label.
Essential is that this shadowing is only applied to paths with a shared prefix $\sgpath$, which corresponds to the prefix order discussed earlier.
\ResolveL~receives a set of labels $\pathlbls$, for which it computes the answer.
It uses two helper functions, defined as follows:
\begin{align*}
  \maxOf{\pathlbls} &\triangleq \setOf{ \pathlbl \in \pathlbls \alt \not\exists \pathlbl' \in \pathlbls.\; \pathlbl \lblOrd \pathlbl' }\\
  \smallerOf{\pathlbls}{\pathlbl} &\triangleq \setOf{ \pathlbl' \in \pathlbls \alt \pathlbl' \lblOrd \pathlbl }
\end{align*}
The $\mathsf{max}$ function returns all labels in $\pathlbls$ for which no greater label exists, and $\mathsf{smaller}$ returns all labels in $\pathlbls$ that are smaller than $\pathlbl$.
Now, \ResolveL~computes its \Lenv as follows.
For each label in the $\mathsf{max}$-set of its $\pathlbls$ argument it computes its \lLenv relative to its $\mathsf{smaller}$-set.
As the \lLenv's of the labels in the $\mathsf{max}$-set are not mutually ordered, the final \Lenv is computed simply by taking their union.

The result of a resolution step is obtained by \ResolveAll, which computes the \Lenv of all path labels that are valid according to $\re'$.
This includes all edge labels that are in its \emph{head set} ($\rehead{\re'}$) and $\EOP$ if the empty word $\varepsilon$ is in the language of $\re'$ ($\langOf{\re'}$).
Finally, the complete query answer is computed by invoking \ResolveAll~with the initial scope as path prefix, and the initial path well-formedness condition.

